Benchmarking Monocular 3D Dog Pose Estimation Using In-The-Wild Motion Capture Data

We introduce a new benchmark analysis focusing on 3D canine pose estimation from monocular in-the-wild images. A multi-modal dataset 3DDogs-Lab was captured indoors, featuring various dog breeds trotting on a walkway. It includes data from optical marker-based mocap systems, RGBD cameras, IMUs, and a pressure mat. While providing high-quality motion data, the presence of optical markers and limited background diversity make the captured video less representative of real-world conditions. To address this, we created 3DDogs-Wild, a naturalised version of the dataset where the optical markers are in-painted and the subjects are placed in diverse environments, enhancing its utility for training RGB image-based pose detectors. We show that using the 3DDogs-Wild to train the models leads to improved performance when evaluating on in-the-wild data. Additionally, we provide a thorough analysis using various pose estimation models, revealing their respective strengths and weaknesses. We believe that our findings, coupled with the datasets provided, offer valuable insights for advancing 3D animal pose estimation.

==> sec/2_relatedwork.tex <==
% \subsection{Related Work}

% \textbf{Model-free vs model-based methods.} Earlier studies on the 3D reconstruction of animals from monocular views had to depend on 2D datasets due to the absence of 3D datasets. These studies can be categorised into two groups: model-based and model-free based methods. 
% %We show in Table X the advantages and disadvantages of both methods. 
% Most of the model-based methods rely on the animal parametric model known as SMAL \cite{Zuffi_2017_CVPR} or a variation of it. For example, together with the Stanford Extra dataset \cite{biggs2020wldo} which includes 12K in-the-wild images and 2D groundtruth labels, has significantly contributed in advancing 3D dog pose/shape estimation research \cite{barc2022rueegg,bite2023rueegg}. 
% %Additionally, parametric models have been used to detect lameness in horses \cite{li2021hsmal}, understand social behaviour in birds \cite{10.1007/978-3-030-58523-5_1} and to observe and track the physical condition and health of livestock animals such as cows \cite{LUO202336}.
% Recently, model-free methods have increased due to the accessibility of internet images and videos, as well as advancements in implicit and neural representations. Initially, much of the work focused on a single category at a time \cite{wu2023magicpony, yao2022lassie}. However, more recently, Li \etal \cite{li2024learning} were able to 3D reconstruct over 100 animal species from internet images by introducing a memory bank regarding semantic information of the animal models.

% While both model-free and model-based methods present their unique strengths and weaknesses in terms of computation, detailed appearance, and occlusion handling, they share common challenges. These include the ambiguity in distinguishing left and right limbs and the uncertainty in depth perception, given their dependence on 2D signals. We strongly believe that 3D datasets would enhance the performance of these methods and therefore propose a 3D dog dataset. 

% \textbf{3D pose datasets}. The majority of existing 3D datasets were acquired in controlled environments using multi-view systems \cite{openmonkey,An2023-qv,Deane_2024_WACV}. The RGBD-Dog dataset \cite{Kearney_2020_CVPR} was captured in a green-screen studio, where dogs were outfitted with motion capture suits. Our research shares similarities with this dataset, as our original data collection took place in a laboratory, where dogs were equipped with optical markers and inertial measurement units (IMUs). Deep learning models trained on this type of RGB data are prone to fail to in-the-wild data as there is a domain gap between the training and real-world data. There has been an effort in producing 3D in-the-wild datasets \cite{Xu_2023_ICCV,10.1109/ICRA48506.2021.9561338} where the 3D ground truth was generated by triangulating the 2D joint coordinates from multiple views. Note that the reliability of the 3D ground truth in these type of datasets is directly tied to the quality of the manual annotations made by humans.

% \textbf{Synthetic datasets}.
%Producing in-the-wild pose datasets is a labour-intensive and complex task, and the accuracy of the 3D ground truth heavily relies on the quality of human annotators. Furthermore, 3D datasets are often confined to controlled environments, rendering them less adaptable for extending 3D reconstruction methods to in-the-wild images. 
% Recognising the limitations associated of producing 3D datasets, previous research have proposed for the creation of synthetic datasets. Various methods exist for generating synthetic datasets, including using real-time game engines \cite{9157335, sydogVid_Shooter} or employing parametric models \cite{Zuffi:ICCV:2019,Xu_2023_ICCV}. However, a major challenge associated with using synthetic training data is the domain gap. %This arises from distinct distributions between synthetic and real data, leading to potential performance issues when deploying models trained on synthetic datasets in real-world scenarios. 
% To address the domain gap, previous research proposed the generation of near-realistic data using style-transfer methods \cite{spac_net} or by modifying the Grand Theft Auto game to simulate real-world data combined by leveraging existing foundation models \cite{Shooter_2024_WACV}.
